Unit Commitment Predictor With a Performance Guarantee: A Support Vector Machine Classifier

The system operators usually need to solve large-scale unit commitment problems within limited time frame for computation. This paper provides a pragmatic solution, showing how by learning and predicting the on/off commitment decisions of conventional units, there is a potential for system operators to warm start their solver and speed up their computation significantly. For the prediction, we train linear and kernelized support vector machine classifiers, providing an out-of-sample performance guarantee if properly regularized, converting to distributionally robust classifiers. For the unit commitment problem, we solve a mixed-integer second-order cone problem. Our results based on the IEEE 6- and 118-bus test systems show that the kernelized SVM with proper regularization outperforms other classifiers, reducing the computational time by a factor of 1.7. In addition, if there is a tight computational limit, while the unit commitment problem without warm start is far away from the optimal solution, its warmly-started version can be solved to (near) optimality within the time limit.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> Revision/Editor.tex <==
\newpage
\section*{\centering{\Large{Response to Editor}}}

% page counter
\setcounter{page}{1}
\renewcommand{\thepage}{E.\arabic{page}}

\begin{center}
	\normalsize
	No. TPWRS-01578-2023 \\
	\textbf{``Unit Commitment Predictor With a Performance Guarantee: A Support Vector Machine Classifier''} \\
	Farzaneh Pourahmadi and Jalal Kazempour
	
	\vskip  0.5 cm	
\end{center}

We thank the editor and three reviewers for their pertinent questions and observations. We have
strived to properly and carefully address all the comments. Detailed answers are provided below.

Please note that reviewer questions are in italics while our answers are not. Additions to the
original manuscript appear in \color{blue} blue \color{black} in both response letter and updated manuscript.

\begin{itemize}
	\setlength\itemsep{1.5em}
	\item [E1)] \textbf{Comment:} \textit{``Comments to the Author:
All the reviewers agree that the topic is timely and interesting. They also raised a few questions for further clarification.''}
	
	\medskip
	\textbf{Response E1:} 
	Thanks for the positive appraisal. In the revised manuscript, all the comments raised by Reviewers 1, 2, and 3 have been thoroughly addressed. We think the current manuscript has
further clarified our contributions, the functioning of the proposed model and its implications. Please see the revised manuscript as well as our detailed response to the following comments. 


 
 	\item [E2)] \textbf{Comment:} \textit{``1. There are many data-driven-based UC research in recent literature. The advantages of SVM compared to existing algorithms should be explained clearly.''}
	
	\medskip
	\textbf{Response E2:} Please see our detailed response to Comment 1 of Reviewer 2. 


 	\item [E3)] \textbf{Comment:} \textit{``2. The issue of how to recover to a feasible solution.''}
	
	\medskip
	\textbf{Response E3:} 
Please see our detailed response to Comment 1 of Reviewer 3.

 	\item [E4)] \textbf{Comment:} \textit{``3. The issue of considering the maintenance of units and transmission lines which are daily tasks in power systems operations.''}
	
	\medskip
	\textbf{Response E4:} 
Please see our detailed response to Comment 2 of Reviewer 1.

 	\item [E5)] \textbf{Comment:} \textit{``4. The statement of Theorem 1 is not clear.''}
	
	\medskip
	\textbf{Response E5:} 
Please see our detailed response to Comment 2 of Reviewer 3.

 	\item [E6)] \textbf{Comment:} \textit{``5. Connection between (8) and (16) should be investigated further.''}
	
	\medskip
	\textbf{Response E6:} 
 Please see our detailed response to Comment 3 of Reviewer 3.

 \item [E7)] \textbf{Comment:} \textit{``6. The 6-bus and 118-bus systems are small and larger systems are required to testify the efficiency of the proposed method.''}

	\medskip
	\textbf{Response E7:} 
Please see our detailed response to Comment 3 of Reviewer 1.

  \item [E8)] \textbf{Comment:} \textit{``7. Clarification of how to generate training data.''}
	
		\medskip
	\textbf{Response E8:} 
Please see our detailed response to Comments 4 and 5 of Reviewer 2.
\end{itemize}

\vspace{0.2cm}

 

==> Revision/Reviewer1.tex <==
\newpage
\section*{\centering{\Large{Response to Reviewer 1}}} \label{sec:Reviewer_1}
% page counter
\setcounter{figure}{0}
\renewcommand{\thefigure}{R1.\arabic{figure}}
\setcounter{table}{0}
\renewcommand{\thetable}{R1.\arabic{table}}
\setcounter{page}{1}
\renewcommand{\thepage}{R1.\arabic{page}}
\setcounter{equation}{0}
\renewcommand{\theequation}{R1.\arabic{equation}}

\begin{itemize}
	\setlength\itemsep{1.5em}
	%
	% 1.1
	\item [1.1)]  \textbf{Comment:} \textit{``The paper is very well organized and prepared. The presentation is very clear and impressive. I must say that I’m happy when I read the manuscript. However, the following important problems need to be clarified.''}
		
	\medskip
	\textbf{Response:} Thank you for your positive feedback. In the revised manuscript, we have added further explanations and extended our case
study by adding further results and supporting discussions.  Please see our detailed response to the following comments raised by the Reviewer.

 	\item [1.2)]  \textbf{Comment:} \textit{``1. Considering the effects of minimum up/down time constraints, the initial on/off states of thermal units are very important when solving a UC problem. How is this problem considered in the proposed method? For example, in the data collection step and in the classification step?''}
		
	\medskip
	\textbf{Response:} \color{black} This is an astute remark. We did not impose any constraint for initial on/off states in generating training and testing datasets, although our proposed framework is general enough to consider different constraints. If we run the UC problem where on/off initial states of conventional units are considered as a constraint for each feature $\mathbf{x}$ and obtain the corresponding UC solution $\textbf{y}$, we can conclude the impact of initial states is included in the data collection step. Then, binary classifiers are trained given this dataset. The only restriction here is that we might need to retrain classifiers for different initial states. Motivated by Reviewer's comment, we have added a new subsection to Section VI.A in the revised manuscript to investigate the impact of initial states. This new subsection reads as follows. 
	\medskip
	
		\textbf{Section VI.A:}
		
\color{blue}{``\textit{Impact of initial states:}
We now investigate the impact of initial states of conventional  units on the accuracy of their commitments' predictions. So far, we have not restricted the initial on/off states of $\rm{G}1$-$\rm{G}3$ in our test system. However, by introducing constraints on the initial states of units in a UC problem, we can compile a dataset that includes the impact of these initial states. Let us suppose that initially,  units $\rm{G}1$-$\rm{G}3$ are all on, represented by $\mathbf{u}_0=[1,1,1]$. We derive the corresponding UC solution $\mathbf{y}$ accordingly to construct our training dataset. Subsequently, we train binary classifiers using this dataset. Fig. \ref{initialstates5_review} shows how accurately the prediction reflects the initial states $\mathbf{u}_0$ considered in the testing dataset, indicating whether they are similar or different from the initial states $\mathbf{u}_0$ considered in the training dataset.

\medskip

The upper plot in Fig. \ref{initialstates5_review} illustrates the accuracy of predictions when the initial states $\mathbf{u}_0$ for testing match with those used in constructing the training dataset. Accuracy here refers to the percentage of incorrect predictions out of $1,000$ testing samples. Additionally, we examine three other scenarios where the initial states $\mathbf{u}_0$ of testing samples differ from those of the training set. We consider four cases only in Fig. \ref{initialstates5_review} as  unit $\rm{G}2$ remains on owed to its lowest operating cost among three units. Therefore, there are $4$ possible combinations of initial states for the two remaining units.

\medskip

From Fig. \ref{initialstates5_review}, we observe that if the initial state of $\rm{G}3$ changes to $0$ during testing, the prediction accuracy remains unaffected. However, for $\rm{G}1$, it is crucial to train binary classifiers specifically for the corresponding initial states. This observation is also valid for larger test systems. Initially, one needs to identify the set of potential initial states and determine which ones require retraining of binary classifiers. It is important to note that all these investigations can be conducted offline.''} 
\begin{figure}
\color{blue}
    \centering
    \includegraphics[width=0.7\columnwidth]{Figures/Initialstates5_cropped.pdf}
    \caption{The accuracy of predictions when the initial states $\mathbf{u}_0$ for testing is different. Accuracy here refers to the percentage of incorrect predictions out of 1,000 testing samples.}
    \label{initialstates5_review}
    \vspace{-1mm}
\end{figure}
 \color{black} 
  	\item [1.3)]  \textbf{Comment:} \textit{``2. It is known that the maintenance of units, transmission lines are also daily task in power systems operations. During the time of maintenance, units/transmission lines are often not considered in the UC problem. This will have no effects for algorithms such as Lagrangian relaxation, Branch-and-cut, and so on since these algorithms do not depend on the historical UC solutions. However, for the proposed method, how to consider this problem? This problem is more serious when N-k security constraints are considered in UC formulation.''}
		
	\medskip
\textbf{Response:} \color{black} Our answer to this comment is in the same line as the previous one. 
 We might need to retrain binary classifiers for any changes in the formulation of the UC problem due to maintenance of conventional units and/or transmission lines. 
 Please note that it is usually the case that the system operator knows a plan for the  maintenance of conventional units and transmission lines in advance like one week before. Therefore, one can safely assume there is enough time to generate training data samples considering the absence of the underlying unit and/or line and retrain the classifiers, accordingly. 

 \medskip
 
We fully agree with the Reviewer that considering $N\!-\!k$ security constraints in the UC problem becomes more serious when some conventional units and transmission lines are in the maintenance phase. We would like to kindly emphasize that our proposed framework is still general enough to include $N\!-\!k$ security considerations. In that case, one would need to add $N\!-\!k$ security constraints into the UC problem, solved for each sample, and follow the same procedure as we discussed before. 

\medskip

For further clarification, we have added the following descriptions to Sections VI and VII of the revised manuscript:


\medskip
	
		\textbf{Section VI:}
		
\color{blue}{``Similarly, for any change in the optimization formulation of
the UC problem, one may need retraining the classifier. This
could be the case when a conventional unit or a transmission
line is out for maintenance, or when the system operator
changes the network topology.''}
 \color{black}

 \medskip
	
		\textbf{Section VII:}
		
\color{blue}{``Additionally,
an intriguing direction for further investigation is to explore
methods for transfer learning to adapt to changes in the UC
problem, such as modifications in network topology, without
a need for retraining the binary classifier.''}
 \color{black}

\item [1.4)]  \textbf{Comment:} \textit{``3. I think 6-bus and 118-bus systems are too small to testify the efficiency of the proposed method. The authors are suggested to test the method on some larger scale systems.''}
		
	\medskip
	\textbf{Response:} \color{black} We share the same view with the Reviewer in case one solves a UC problem with linearized DC power flow equations as it is common in the literature. Please recall that this work solves the UC problem with relaxed AC power flow equations, resulting in a mixed-integer second-order cone programming (MISOCP) problem, which brings way more computational burden than classical UC problems as a mixed-integer linear program (MILP). Our intention for such a choice is to model UC problem as close as possible to real world without using such a highly approximated linearized DC power flow model. Despite all recent advances in MISOCP solvers such as Gurobi, they are still way slower than their MILP counterparts. Please let us kindly provide the Reviewer with some computational considerations: To generate the training dataset for 118-bus test system, we need to solve a MISOCP problem with 2,592 binary variables, 13,920 continuous variables, and 55,464 linear and conic constraints for each sample. This is already a large-scale  optimization problem for state-of-the-art MISOCP solvers. Consequently, the computational demands become prohibitively high when considering systems larger than the 118-bus system. In our investigation of related literature on the UC problem with AC power flow \cite{UC_AC1,UC_AC2,UC_AC3,UC_AC4,UC_AC5}, 
 we found out that the largest systems considered in similar studies is of a comparable scale to the 118-test system.

	\medskip
 
Alternatively, one could opt to address the UC problem using a mixed-integer linear program. However, the advantage offered by our proposed framework becomes less pronounced in such cases. For instance, when we solve the UC problem with DC power flow on a case with 1,888 buses, 297 generating units, and 2,531 transmission lines, the computational time is around 300 seconds. Consequently, there is no  need for warming up the solver in such cases. To address the Reviewer's comment, we have added the following footnote to Section VI.B of the revised manuscript:\color{black}

 \medskip
	
\textbf{Section VI.B:}
		
\color{blue}{``We realize the computational requirements are way more significant when
solving MISOCP problem for cases larger than the 118-bus test system. In the
relevant UC literature including AC power flow equations [3], [44]–[47], we
found out that the largest system considered in those studies is of a comparable
scale to the 118-test system.''}
 \color{black}

 
 \end{itemize}
	

==> Revision/Reviewer2.tex <==
\newpage
\section*{\centering{\Large{Response to Reviewer 2}}} \label{sec:Reviewer_1}
% page counter
\setcounter{figure}{0}
\renewcommand{\thefigure}{R2.\arabic{figure}}
\setcounter{table}{0}
\renewcommand{\thetable}{R2.\arabic{table}}
\setcounter{page}{1}
\renewcommand{\thepage}{R2.\arabic{page}}
\setcounter{equation}{0}
\renewcommand{\theequation}{R2.\arabic{equation}}

\begin{itemize}
	\setlength\itemsep{1.5em}
	%
	% 1.1
	\item [2.1)]  \textbf{Comment:} \textit{``Comments to the Author}
 
\textit{This paper proposed a support vector machine model to warm start unit commitment computation. The topic is of interest and timely. The reviewer has the following questions.''}
		
	\medskip
	\textbf{Response:} Thanks for the positive appraisal. Please see our detailed response to the following comments raised by the Reviewer. 

 	\item [2.2)]  \textbf{Comment:} \textit{``1. There are many data-driven-based UC research in recent literature. The advantages of SVM compared to existing algorithms should be explained clearly. The contributions and innovations should be better clarified.''}
		
	\medskip
	\textbf{Response:} 
 Thanks for this pertinent comment. We have provided a comprehensive literature review on data-driven UC approaches in the revised manuscript. Given this extended literature review, we think  our contributions and the advantages of our proposed binary classifiers are now clearer. Please see our changes below: 
 \medskip
	
		\textbf{Section I:}
		
\color{blue}{``\textit{A. Literature review}


Several studies in the literature propose various solutions to reduce the computational complexity of the deterministic
UC problem expressed as a mixed-integer linear program.
Techniques employed include formulation tightening [11]–[14], decomposition techniques [15], and constraint screening
[16]. However, they overlook the fact that the same UC
problem with (slightly) different input data is being solved
regularly.

A key that may give the system and market operators an
advantage is that they solve the UC problem every day, and
therefore they usually have access to an extensive historical
database of UC solutions under various operational circumstances. This may enable the operators to speed up the com-
putation process by learning from previous solutions. With the
recent advances in the field of machine learning, it is promising
to learn from previous data to ease the computational burden.
Exploiting machine learning techniques to accelerate the rate
at which mixed-integer convex optimization problems are
solved is a relatively new research field [17], particularly
in the context of power systems. We have identified three
strands in literature that use machine learning techniques for
power system optimization, and more specifically for the UC
problem.


The first strand aims to develop so-called surrogate or
optimization proxies, for which an estimator function is used
to learn a direct mapping between contextual information,
i.e., features, such as the forecast of demand and renewable
production, and the optimal operational schedules [18], [19]. In
the context of the UC problem, [20] and [21] develop a proxy
for the UC solution by learning a direct mapping between
features and optimal unit commitments.


The second strand develops so-called indirect models,
wherein an estimator function maps features to some infor-
mation to reduce the optimization problem dimension. This
information could be the prediction of active constraints and/or
the value of some (binary) variables. This reduces the com-
plexity of the original optimization problem in terms of the number of constraints and/or binary variables by eliminating
inactive constraints and/or setting binary variables to predicted values [22]–[25]. In the context of the UC problem, [26]–[28] learn the optimal value of unit commitments and active con-
straints to reduce the dimension of the optimization problem
formulated as mixed-integer linear program.


The main drawback of the first two strands is that they
may fail to correctly predict the optimal solution. One of the
main causes of this shortcoming is that they are unable to use
pre-existing mathematical form of the optimization problem
as they completely replace existing optimization models by
machine learning proxies. Although in the second strand, a
(reduced) optimization problem is solved to find a solution, a
feasibility and optimality guarantee might be still missing.


The third strand develops an estimator function, predicting
the value of some variables as a starting point called a
warm start to speed up the solution process of non-linear or
mixed-integer problems [29]–[31]. The main advantage of this
technique is that, depending on the type of the underlying
optimization problem, the feasibility and likely optimality of the solution can still be guaranteed, while the problem is
being solved faster. Nevertheless, the disadvantage is that there
might be cases under which a warm start brings insignificant
computational benefit or even increases the computational time
in an extreme case. Among others, this may happen if the
warm start suggests an initial solution which is infeasible or
far from the optimal point. Therefore, reducing the solution
time depends on the accuracy of warm start. Furthermore,
the learning-based data-driven methodologies in the context
of power systems overlook how to build an efficient training
dataset and generalized learning in the case of unseen data
with a performance guarantee.''} 
\color{black}




\color{black}

  	\item [2.3)]  \textbf{Comment:} \textit{``2. The AC power flow usage in the UC problems should be explained. Although ACPF can obtain more feasible power flow solutions, existing UC models usually use DC-based power flow. The conic relaxation of AC power flow in the transmission network might not obtain optimal solutions.''}
		
	\medskip
	\textbf{Response:} \color{black}
 We do agree with the Reviewer that the majority of existing models for the UC problem is formulated as a mixed-integer linear program, utilizing the linearized DC power flow equations to alleviate computational complexity. However, the drawback of models with DC optimal power flow equations, as highlighted in \cite{KyriBaker}, is that their solutions are \textit{never} compatible with AC systems. With recent advances in mixed-integer solvers, we think that optimization models including convexified but nonlinear AC  power flow equations are becoming more tractable problems, making the previous emphasis on DC power flow for fast computation less compelling.


	\medskip
 
Although utilizing the conic relaxation with AC optimal power flow may not always yield an optimal \textit{yet} feasible solution (depending on the relaxation gap), as demonstrated in \cite{UC_AC3}, it has been shown that the DC UC problem is even worse, as its solution is always infeasible to AC systems. 
%whereas formulating the AC UC problem as a mixed-integer second-order cone programming (MICOCP) problem provides AC feasible solutions with small optimality gaps. 
%Through various examples, it has been consistently demonstrated that the MISOCP-based approach outperforms the DC-based approach. 
To properly address the Reviewer's comment, we have provided a justification for the use of relaxed AC power flow equations in the revised manuscript as follows:

\medskip
	
		\textbf{Section II:}
		
\color{blue}{``For the UC problem formulation, we opt for AC power flow over linearized DC power flow
equations since the solutions of DC power flow are never AC
feasible [32]. Aiming to include the AC power flow equations
while keeping the convexity (needed for keeping the problem
tractable with binaries), we use a UC formulation with the
conic relaxation of AC power flow [33], resulting in a mixed-
integer second-order cone programming (MISOCP) problem.''}
 \color{black}

\item [2.4)]  \textbf{Comment:} \textit{``3. The network power flow and commitment solutions depend not only on the renewable and demand forecast, but they also depend on the network topology and energy prices. Should this information be used in the training data set? The topology changes are not uncommon in daily operation which should be considered.''}
		
	\medskip
	\textbf{Response:} \color{black} 
 
It is indeed accurate that both network power flow and commitment solutions are influenced by the network's topology. Please refer to our response to Comments 1 and 2 of Reviewer 1 which are similar to this comment. For any changes in the optimization formulation of the UC problem, one will need to retrain the proposed binary classifiers. Since the range of potential network topologies is finite and limited, we can compile the corresponding dataset and train binary classifiers \textit{offline}, accordingly. %With knowledge of the system's topology a day in advance, we can utilize these classifiers to predict the UC solution.

\medskip
Regarding energy prices, we approach the UC problem   from the system operator's perspective without market considerations. The operator executes the UC problem to clear the market and establish energy prices. Therefore, energy prices emerge as the output of solving the UC problem. Therefore, it is not necessary to consider them as inputs to the UC problem. Consequently, the UC solutions remain independent of energy prices. Various techniques exist for pricing energy based on the UC problem [1]-[2], which fall beyond the scope of the current work.

\medskip

For further clarifications, we have added the following descriptions to the revised manuscript:


\medskip
	
		\textbf{Section VI:}
		
\color{blue}{``Similarly, for any change in the optimization formulation of
the UC problem, one may need retraining the classifier. This
could be the case when a conventional unit or a transmission
line is out for maintenance, or when the system operator
changes the network topology.''}
 \color{black}

 \medskip
	
		\textbf{Section VII:}
		
\color{blue}{``Additionally,
an intriguing direction for further investigation is to explore
methods for transfer learning to adapt to changes in the UC
problem, such as modifications in network topology, without
a need for retraining the binary classifier.''}
 \color{black}
 
\medskip
	

[1] N. Azizan, and et al., "Optimal pricing in markets with nonconvex costs", Operations Research, vol. 68, no. 2, 2020.

\medskip
[2] RP. O’Neill, and et al., "Efficient market-clearing prices in markets with nonconvexities", Eur. J. Oper. Res, 2005.

\item [2.5)]  \textbf{Comment:} \textit{``4. In the case study, how the training data was generated should be explained. Using random generation or with some historical data? The patterns in the input renewable and demand data should be briefly mentioned.''}

 \item []  \textbf{Comment:} \textit{``5. How was the number of training and testing data scenario determined? Was there any metric for this?''}
		
	\medskip
	\textbf{Response:} 
We found Comments 4 and 5 interrelated, therefore we decided to address them together. While our samples were randomly generated, we designed the training dataset strategically to ensure a sufficient number of samples, guaranteeing an upper bound on the probability of encountering a new commitment solution. The minimum number of training samples, denoted as $H$, is determined using Theorem 1 in the manuscript. Assuming a desired probability guarantee, $\delta$, with a confidence level of $1-\epsilon$, we select $H$ samples to satisfy the following inequality:

\begin{equation}
    \frac{H_1}{H} + (2\sqrt{2}+\sqrt{3}) \sqrt{\frac{1}{H}ln(\frac{3}{\epsilon})} > \delta,
\end{equation}
where $H_1$ represents the count of unique commitment solutions observed. The left side of the equation estimates the probability of encountering a new commitment solution, while the right side provides the upper bound guarantee. Further clarification on this can be found in our response to Comment 2 of Reviewer 3. As for the number of samples in the testing dataset, there are no limitations.

\medskip
Regarding the feature patterns, we assume a consistent daily load and wind power generation profile across samples, with variation only in their levels. Additionally, we presume all loads and wind farms adhere to a fixed power factor. For example, in the IEEE 6-bus test system, to enhance visualization, we consider deterministic loads and stochastic generation for two wind farms, resulting in only two features. To conduct bias analysis for this system, we create a training dataset with 5,000 samples and two distinct testing datasets, each comprising 1,000 samples. One testing dataset closely resembles the training dataset and is termed biased, while the other one differs more and is termed unbiased. Fig. \ref{correlation_review} presents a matrix of plots for the training and two testing datasets separately. Diagonal plots illustrate wind production level histograms, whereas scatter plots depict the correlation between the two wind farms. As observed in Fig. \ref{correlation_review}, the biased test dataset closely resembles the unbiased testing dataset in terms of mean, standard deviation (std.), and correlation coefficients of the two wind farms.

\medskip
To address these two comments, we have added further clarifications to the revised manuscript as follows:
\medskip
	
		\textbf{Section VI:}
		
\color{blue}{``Fig. \ref{correlation_review} presents a matrix of plots for the training and two biased and unbiased testing datasets separately. Diagonal plots illustrate wind production level histograms, whereas scatter plots depict the correlation between the two wind farms. As observed in Fig. \ref{correlation_review}, the biased testing dataset closely resembles the unbiased one in terms of mean, standard deviation (std.), and correlation coefficients of the two wind farms.''}

\begin{figure}
    \color{blue}\centering
    \includegraphics[width=0.7\columnwidth]{Figures/correlationmatrix3_cropped.pdf}
    \caption{A matrix of plots for the training dataset and biased and unbiased
testing datasets. The diagonal plots (x-axis: in per-unit; y-axis: frequency of
occurrence) display the wind production level frequency. The off-diagonal
plots (both axes in per-unit) display the correlation of two wind farms W1-
W2.}
    \label{correlation_review}
    \vspace{-1mm}
\end{figure}
 \color{black}



 

\item [2.6)]  \textbf{Comment:} \textit{``6. Comparisons to other state-of-the-art methods should be included to benchmark the advantages.''}
		
	\medskip
	\textbf{Response:} 
        This is a very valid and constructive comment. We have implemented a k-nearest neighbors (KNN) method, exploited in \cite{Juanmi} and \cite{xavier} for the UC classification, as the benchmark. The implementation process and our observations are described as follows in the revised manuscript:  
        
        %Considering the literature on learning-based data-driven methodologies in the context of the UC problem which is discussed in response to Comment 1, we found out models proposed in \cite{Juanmi} and \cite{xavier} are more relevant and comparable to this work. The work \cite{Juanmi,xavier} employs a classical supervised learning method called k-nearest neighbors (KNN) to predict the commitment of generating units. Consequently, we adopt KNN as a benchmark for constructing binary classifiers and compare its prediction performance with that of SVM techniques. Furthermore, the authors in \cite{Juanmi} claim that the performance of existing and upcoming learning-based methods to solve the UC problem should be compared with some simpler and straightforward, yet effective methods like KNN. Inspired by this viewpoint, we treat KNN as a benchmark and investigate the effectiveness of both KNN and SVM in predicting the correct commitments.

%\medskip
%The rationale behind KNN is to identify the most similar examples in the training dataset and to conduct a majority vote. Specifically, for a given feature vector $\Tilde{\mathbf{x}}$, the method sorts the training dataset $(\mathbf{X,Y})$ based on increasing distances $||\mathbf{x}_h-\Tilde{\mathbf{x}}||_2$ for all $h=1,..,H$. Subsequently, it selects the first k nearest neighbors to $\Tilde{\mathbf{x}}$ with the lowest distances, denoted as $\{(\mathbf{x}_1,\mathbf{y}_1),..,(\mathbf{x}_k,\mathbf{y}_k)\}$. Then, to predict each binary variable $\Tilde{y}_{gt}$, we compute the average of the values $\frac{y_{1gt}+...+y_{kgt}}{k}$. If the average is positive, $\Tilde{y}_{gt}=1$; otherwise, $\Tilde{y}_{gt}=-1$. It's worth noting that similar to SVM, we map $\Tilde{y}_{gt}=-1$ back to $\Tilde{y}_{gt}=0$.


%Initially, we implement the KNN method on the IEEE 6-bus test system. Please see our changes in Section VI.A as follows:

\medskip
	
		\textbf{Section VI.A:}
		
\color{blue}{``\textit{Benchmark model}: We have found models developed in
\cite{Juanmi} and \cite{xavier} relevant and comparable to the UC predictor
proposed in this work. They employ a classical supervised
learning method called k-nearest neighbors (KNN) to predict
the commitment of conventional units. We adopt KNN as
a benchmark for constructing binary classifiers and compare
its prediction performance with that of the proposed SVM
classifiers. Furthermore, \cite{Juanmi}  concludes that the performance of existing and upcoming learning-based methods to solve the UC problem should be compared with some simple and
straightforward, yet effective methods like KNN. Inspired by
this viewpoint, we treat KNN as a benchmark and investigate
the effectiveness of both KNN and SVM classifiers in predicting the correct commitments.

\medskip
The rationale behind KNN is to identify the most similar examples in the training dataset and conduct a majority vote. Specifically, for a given feature vector $\Tilde{\mathbf{x}}$, the method sorts the training dataset $(\mathbf{X,Y})$ based on increasing distances $||\mathbf{x}_h-\Tilde{\mathbf{x}}||_2$ for all $h=\{1,...,H\}$. It selects the first $k$ nearest neighbors to $\Tilde{\mathbf{x}}$ with the lowest distances, denoted as $\{(\mathbf{x}_1,\mathbf{y}_1),...,(\mathbf{x}_k,\mathbf{y}_k)\}$. Then, to predict each binary variable $\Tilde{y}_{gt}$, it computes the average of the values $\frac{y_{1gt}+...+y_{kgt}}{k}$. If the average is positive, $\Tilde{y}_{gt}=1$; otherwise, $\Tilde{y}_{gt}=-1$. It is worth noting that similar to SVM, we map $\Tilde{y}_{gt}=-1$ back to $\Tilde{y}_{gt}=0$.

\medskip
Consider plot 12 in Fig. 3, illustrating the classification
boundary generated by Kernelized SVM for the commitment
of a randomly chosen conventional unit G3 during a specific
hour. We then apply the KNN technique to this particular
example to determine its classification boundary. It is worth
mentioning that we have employed a cross-validation approach to fine-tune the parameter k in the KNN technique. A
comparison between SVM and KNN boundaries is depicted
in Fig. \ref{KNN_SVM_Review}. In both cases, 14 out of 1,000 test samples are
misclassified. We repeat this process for other binary classifiers
corresponding to different units and hours, observing that
SVM and KNN exhibit almost identical performance. This observation confirms the conclusion in \cite{Juanmi}, stating that KNN might work satisfactory for the UC classification such that more complex classifiers might be unnecessary. However, we realize that it holds true for this small-scale 6-bus test system. In the next section with a larger case study, we will observe that the proposed SVM classifier outperforms KNN by a system cost saving of  $5\%$ when there is a time limit for the computation task or  a computational time reduction of $3\%$ when there is no such a limit.''}

\begin{figure} \color{blue}
    \centering
    \includegraphics[width=0.7\columnwidth]{Figures/svm_knn_plot-compressed_new.pdf}
    \caption{Comparison of Kernelized SVM with regularization and KNN classifiers.}
    \label{KNN_SVM_Review}
    \vspace{-1mm}
\end{figure}

 \medskip
\color{black}
We also implemented the KNN technique for IEEE 118-test system. We have added another subsection to Section VI.B as follows:

 \medskip
	
		\textbf{Section VI.B:}
		
\color{blue}{``\textit{Benchmark model}: We employ KNN predictions as a warm start for the MISOCP problem. Similar to our approach in evaluating different SVM techniques, we explore two scenarios to assess KNN's prediction effectiveness in reducing computational costs. In scenario I, constrained by a computational time limit of $700$ seconds, the system cost using KNN predictions as a warm start is $\$277,010$. 
The kernelized SVM continues to provide more effective warm starts, resulting in a $5\%$ improvement compared to KNN. In scenario II, where there are no computational time constraints, utilizing KNN predictions as a warm start allows solving the UC problem to optimality with an expected computational time of $1,354$ seconds. Warm starting with kernelized SVMs reduces the computational time by $3\%$ compared to KNN.''}
\color{black}
 
 
 \end{itemize}


==> Revision/Reviewer3.tex <==
\newpage
\section*{\centering{\Large{Response to Reviewer 3}}} \label{sec:Reviewer_1}
% page counter
\setcounter{figure}{0}
\renewcommand{\thefigure}{R3.\arabic{figure}}
\setcounter{table}{0}
\renewcommand{\thetable}{R3.\arabic{table}}
\setcounter{page}{1}
\renewcommand{\thepage}{R3.\arabic{page}}
\setcounter{equation}{0}
\renewcommand{\theequation}{R3.\arabic{equation}}

\begin{itemize}
	\setlength\itemsep{1.5em}
	%
	% 1.1
	\item [3.1)]  \textbf{Comment:} \textit{``This manuscript proposes a support vector machine (SVM) to predict a good feasible unit
commitment (UC) decision vector, which can be used as a warm-start of branch-and-bound type algorithms. The key simplification is to train an SVM for each generator in each time period.
Upon this idea, both linear and kernelized SVM are proposed, as well as regularization (or what is claimed to be the distributionally robust formulation) to enhance the prediction quality.
Numerical experiments based on IEEE 6-bus and 118-bus systems are included to show the effectiveness of the prediction in accelerating and improving the UC solution within certain time limits.}


\textit{The reviewer finds the topic of this manuscript interesting and fit for this journal. However, the reviewer also finds that some very important details are missing in the current version and a few changes in the presentation are suggested for clarity and rigor.''}
		
	\medskip
	\textbf{Response:} Thanks for thorough summary. Please see our detailed response to the following comments raised by the Reviewer.

 	\item [3.2)]  \textbf{Comment:} \textit{``1. In the (possibly biased) opinion of the reviewer, the most important step is to ensure the
feasibility of the prediction. Regarding this, the authors have mentioned a few times that they are using the k-nearest neighbor search to recover a feasible UC decision from an infeasible one, without, however, spending any paragraph on describing the details of it. As there  does not seem to be any guarantee of the SVM ensuring the min-up and min-down constraints (not to mention power flow feasibility), the reviewer believes that the feasibility recovery could critically impact the effectiveness of the proposed method.''}
		
	\medskip
	\textbf{Response:} Thanks for bringing up this pertinent concern. As the Reviewer correctly pointed out, there is no guarantee that SVM can ensure the minimum up and down-time constraints. Therefore, a procedure for recovering feasibility might be necessary. Please find our adjustments outlined below. As the approach we use for the feasibility recovery is different from the KNN algorithm that we added to the revised manuscript in response to Comment 6 of Reviewer 2, we now refer to our feasibility recovery approach as a heuristic to prevent any confusion. In response to this comment, our additions to the revised manuscript are as follows:

 \medskip
	
		\textbf{Section II:}
		
\color{blue}{``If the prediction is undesirable
due to infeasibility, we first recover a feasible solution from
the sampled strategies to the infeasible one using a heuristic
approach, and then use it as a warm start to the original UC
problem.''}
\color{black}

 \medskip
	
\textbf{Section V:}
		
\color{blue}{``Recall that the predicted $\tilde{\mathbf{y}}$ to be used as a warm start might be infeasible for the MISOCP problem. 
If $\tilde{\mathbf{y}}$ is infeasible since it fails to meet the minimum up- and down-time constraints, we find a close feasible solution among the sampled strategies to the infeasible one by using a heuristic approach to recover a feasible solution. The heuristic approach sorts 
 the training dataset $(\mathbf{X,Y})$ based on increasing distances $||\mathbf{y}_h-\Tilde{\mathbf{y}}||_2$ for all $h=\{1,...,H\}$. Then, it selects the nearest $\mathbf{y}_h$ to $\tilde{\mathbf{y}}$ represented by $\hat{\mathbf{y}}$ to be used as a warm start. In the case where there are multiple $\hat{\mathbf{y}}$ having the same distance to $\tilde{\mathbf{y}}$, we can select the one that occurs the most in the training dataset. Knowing $\mathbf{y}_h$ for all $h=\{1,...,H\}$ satisfies the minimum up- and down-time constraints, the warm start $\hat{\mathbf{y}}$ meets these constraints as well. Furthermore, in order to guarantee that there is always a feasible solution to the UC problem in terms of satisfying power flow constraints, we also take extreme corrective measures such as load shedding and renewable power curtailment into consideration.''}
\color{black}

 \medskip
\textbf{Section VI:}
		
\color{blue}{``If $\tilde{\mathbf{y}}$ is not binary feasible, we find a feasible strategy that is as close as possible to the predicted strategy among the strategies sampled for training dataset.''}
\color{black}



  	\item [3.3)]  \textbf{Comment:} \textit{``2. The statement of Theorem 1 is not clear to the reviewer. In particular, what is the
"corresponding set of strategy vectors $\mathbf{Y}$"? Apparently it cannot be all possible strategies because there could be unobserved strategy vector $\mathbf{y}_{H+1}$. Moreover, the meaning of $\mathbf{H}_1$ and $\epsilon$ may need further clarification as well. While the proof "can be directly derived" from
the literature, it is still suggested that the authors include a short proof/explanation, or cite
the original statement in the literature in the appendix. This could greatly help readers' understanding.''}
		
	\medskip
	\textbf{Response:} 
 Thanks for this pertinent suggestion. We have added further clarifications on Theorem 1. Please see the following additions:

 	\medskip
 		\textbf{Section III:}
		
\color{blue}{``This theorem provides us with an approach to estimate the probability of observing an unseen set of commitment decisions. 
Let us delve deeper into this theorem. Consider a set of commitment solutions, denoted as $\mathbf{Y}$, with a total of $H$ solutions. Let $\mathbf{Y}_k$ denote the subset of commitment solutions occurring exactly $k$ times within $\mathbf{Y}$. We use $M_k$ to represent the probability of observing a commitment solution $k$ times. Good-Turing estimators, denoted as $G_k$, provide estimates for $M_k$ as 
\begin{equation}
    G_k=\frac{k+1}{H-k}|\mathbf{Y}_{k+1}|, 
\end{equation}
where $|\cdot|$ denotes the size of a set. In particular, the estimator $G_0$ for observing unseen commitment solutions is given by $G_0=\frac{|\mathbf{Y}_{1}|}{H}$. We denote $|\mathbf{Y}_{1}|$ as $H_1$, representing the count of unique commitment solutions or strategies. Intuitively, when there are numerous different commitment solutions but a relatively small training dataset, the estimate of $M_0$ may be 1. This scenario can occur when collecting a large number of training samples is computationally burdensome. Therefore, $G_0$ is not a good estimate of $M_0$. In order to resolve this problem, [34] establishes a bound on the bias of the Good-Turing estimator $G_0$ and extends it using confidence notations. It provides a tight upper bound on the special case of $M_0$ with a confidence level of $1-\epsilon$, expressed as

\begin{equation} 
    M_0 \leq \frac{H_1}{H} + (2\sqrt{2}+\sqrt{3})\sqrt{\frac{1}{H}ln(\frac{3}{\epsilon})}.
\end{equation}  

In other words,  (R1.2) is satisfied with a probability of at least $1-\epsilon$ over the choice of samples. Considering this theorem, we keep sampling until the bound on the right-hand side of (R1.2) falls below a desired probability guarantee of $\delta$ with a given confidence interval of $1-\epsilon$. This strategy sampling is detailed in Algorithm 1.''}
\color{black}
 
 
 \color{black}

\item [3.4)]  \textbf{Comment:} \textit{``3. Equations (8) and (16) are the regularized versions of the SVM and are claimed to be equivalent to the distributionally robust formulation, so the authors spend multiple
paragraphs to explain the latter. The issue is that unlike the classical regularization, as cited from [1], the Tikhnonov regularization used in this manuscript does not have a direct equivalence and thus requires another unknown parameter , which can be very different from the radius . In fact, in the numerical experiments, the authors directly choose the
regularization parameter directly through cross validation without any reference of the radius . In this regard, the reviewer believes that the connection of (8) and (16) to distributionally robust formulation is only theoretical (which is fine), but slightly misleading in
the current presentation. The reviewer thus suggests that the authors shorten the
unnecessary description of the distributionally robust formulation to leave space for more important explanations, as pointed out in the above comments.''}
		
	\medskip
	\textbf{Response:} We do agree with the Reviewer that there is no explicit formulation to link the radius and the regularization parameter. Motivated by the Reviewer's comment, we have shortened the parts related to distributionally robust classifiers to leave space for the further explanation of Theorem 1. Please see Sections IV.D and IV.E in the revise manuscript, which read as follows:

	\medskip
\textbf{Section IV.D:}
		
\color{blue}{``\textit{Distributionally robust  SVM}

The literature often assumes that training and test datasets follow the same distribution, however this is not necessarily a valid assumption. When the distribution of training data is unknown, it is helpful to create a classifier which is robust to distributional uncertainty. One potential method is to use a Wasserstein distributionally robust optimization, yielding a distributionally robust SVM.

Built upon \eqref{SVM_regularized_continous}, the distributionally robust  SVM writes as
\begin{align} \label{DRC_linear_review}
\min_{\mathbf{w},b}& \ \sup_{\mathbb{Q}\in \mathbb{B}_\rho(\hat{\mathbb{P}}_H)} \mathbb{E}^\mathbb{Q} \bigg[\mathbf{L}\big(y,(\mathbf{w}^\top \mathbf{x}+ b )\big)\bigg],
\end{align} 

where $\mathbb{B}_\rho(\hat{\mathbb{P}}_H)$ denotes the set of distributions, whose distance to the empirical distribution $\hat{\mathbb{P}}_H$ is lower than or equal to the pre-defined value $\rho\in \R$. Optimization \eqref{DRC_linear_review} obtains the worst distribution $\mathbb{Q}$ within $\mathbb{B}_\rho(\hat{\mathbb{P}}_H)$, and optimally classifies samples against it. It has been proven in \cite{Soroush1} and \cite{Soroush2} that, under certain circumstances, \eqref{DRC_linear_review}  is equivalent to a \textit{regularized} version of the linear SVM \eqref{SVM_regularized_continous_review}. 
%
%A comprehensive characterization of the circumstances under which DRC and regularization are equivalent has been outlined in \cite{Soroush1} and \cite{Soroush2}. We here stick into the SVM classifier, since its corresponding loss function, i.e., the hing loss function, is convex and Lipschitz continuous. Therefore, we tractably reformulate (\ref{DRC_linear}). It has been elaborated in \cite{Soroush1} and \cite{Soroush2} that DRC problems utilizing SVM with a hing loss function can be considered analogous to a classical regularized SVM, if there is no uncertainty in the outputs. In such cases, any distribution that is close to the empirical distribution of the training data can diffuse the features, but it cannot change the strategies from $+1$ to $-1$ or vice versa. Thus, classical regularization schemes implicitly assume that output measurements are exact. 
%
%To satisfy those circumstances, we make an assumption that only the underlying distribution of features $\mathbf{x}$ is unknown. By this, the 2-Wasserstein 
%By this, the radius $\rho$ is equivalent to the regularization weight parameter $\lambda$, such that 
Accordingly, for every $\rho \ge 0$, there exists a value $\lambda\in \R$ such that the distributionally robust  SVM is analogous to the regularized  SVM. 
%Similar to classical classification, the regularization parameter can be obtained by a cross validation. 
As a result, \eqref{DRC_linear_review} is equivalently rewritten as
\begin{align} \label{SVM_DRC_regularized_review}
\min_{\mathbf{w},\mathbf{b}}& \ \frac{1}{H}  \sum_{h=1}^H \mathbf{L}\big(y_h,(\mathbf{w}^\top \mathbf{x}_h+b )\big)+\lambda \lVert \mathbf{w} \rVert ^2_2,
\end{align} 
%formulation (\ref{SVM_regularized_kernel}) can be considered as distributionally robust classifier. 
where  $\lVert \cdot\rVert_2$ is the $2$-norm. The second term in (\ref{SVM_DRC_regularized_review}) is the regularization term to avoid over-fitting. 
%Note that (\ref{SVM_DRC_regularized}) is an unconstrained quadratic programming (QP) problem.
The resulting distributionally robust SVM offers an upper-bound guarantee on the expected prediction loss function, commonly referred to as an out-of-sample guarantee.
Let us consider a test dataset $\{(\Tilde{\mathbf{x}}_1,\Tilde{y}_1),...,(\Tilde{\mathbf{x}}_h,\Tilde{y}_h),...,(\Tilde{\mathbf{x}}_{\Tilde{H}},{\Tilde{y}}_{\Tilde{H}})\}$ of $\Tilde{H}$ samples. Assuming the distribution of the test dataset lies in $\mathbb{B}_\rho(\hat{\mathbb{P}}_H)$, it holds that
%the following generalization bounds on the out-of-sample prediction loss holds with the probability of $1-\eta$.
%
\begin{align} \label{predictionguarantee_linear_review}
 \frac{1}{\Tilde{H}} \sum_{h=1}^{\Tilde{H}} \mathbf{L}\big(\Tilde{y}_h,(\mathbf{w^{*}}^\top \Tilde{\mathbf{x}}_h+ b^{*} )\big)  \leq J(\lambda),
\end{align}
%where $1-\eta$ is also the probability that the distance between the distribution of test data and that of training data is less than the Wasserstein radius. 
where $J(\lambda)$ is the optimal value of (\ref{SVM_DRC_regularized_review}). 
%The takeaway is that the distributionally robust SVM (\ref{SVM_DRC_regularized}) is equivalent to the regularized form of the linear SVM \eqref{Linear_SVM_1}, i.e., 
%
Problem (\ref{SVM_DRC_regularized_review}) can be efficiently solved by replacing $\lambda \lVert \mathbf{w} \rVert ^2_2 $  by an auxiliary variable $\varrho$ as
%
%and then adding the constraint $\varrho \geq \lambda \lVert \mathbf{w} \rVert ^2_2$.
\begin{subequations} \label{Linear_SVM_2_review}
\begin{align} 
\min_{\zeta_h \geq 0,\mathbf{w},b}& \ \ \frac{1}{H} \sum_{h=1}^H \zeta_h + \varrho \\
     \text{s.t.} \  \ & y_h (\mathbf{w}^\top \mathbf{x}_h+ b) \ge 1-\zeta_h, \ \forall h \\
     & \varrho \geq \lambda \lVert \mathbf{w} \rVert ^2_2.
     \label{soft_review}\
\end{align}
\end{subequations}
 
 
 By doing so, \eqref{Linear_SVM_2_review} becomes a second-order cone programming (SOCP) problem with a linear objective function.''}
\color{black}

\medskip
\textbf{Section IV.E:}
		
\color{blue}{``\textit{Distributionally Robust Kernelized SVM}

Similar to the discussion for \eqref{DRC_linear_review}, it has been proven in \cite{Soroush1}  and \cite{Soroush2} that the kernelized SVM  
%\eqref{SVM_DRC_regularized_kernel} 
with the regularization term $\lambda \lVert {\boldsymbol{f}^{\frac{1}{2}}\boldsymbol \beta} \rVert ^2_2$, under certain conditions, is equivalent to a distributionally robust kernelized classifier as
%
\begin{align} \label{DRC_nonlinear_review}
\min_{\boldsymbol\beta}& \sup_{\mathbb{Q}\in \mathbb{B}_\rho(\hat{\mathbb{P}}_H)} \mathbb{E}^\mathbb{Q} \Big[\mathbf{L}\Big(y,\sum_{h=1}^H   f(\mathbf{x},\mathbf{x}_h) \beta_h\Big)\Big].
\end{align}

Similar to \eqref{predictionguarantee_linear_review}, it holds that
\begin{align}
 \frac{1}{\Tilde{H}} \sum_{k=1}^{\Tilde{H}} \mathbf{L}\Big(\Tilde y_k,\sum_{h=1}^H   f(\Tilde{\mathbf{x}}_k,\mathbf{x}_h) \beta^{*}_h\Big) \leq J'(\lambda),
\end{align}
where $J'(\lambda)$ is the optimal value of \eqref{dual_kernel_primal}.''}
\color{black}
 

\item [3.5)]  \textbf{Comment:} \textit{``Below are some other suggestions for the authors to consider.}


\textit{Many MISOCP solvers such as Gurobi uses random seeds and parallel computing, which
creates uncertainty in the obtained solutions especially within time limits. Thus the reviewer suggests further clarification (on whether they have disabled any randomization and tried to
eliminate such uncertainty), or more precise definitions (such as "* refers to the optimal value obtained by the state-of-the-art solvers" above Theorem 1, which is vague as there could be different solutions depending on the randomization).''}
		
	\medskip
	\textbf{Response:} Thank you for your insightful comment.  By the optimal value obtained by advanced solvers like Gurobi, we refer to the value achieved when we run the solver without any time constraints. We have noticed that even after running the solver several times, we end up in the same solution. However, in the cases where we have enforced a time limit, we may end up in different solutions but not for the cases where we warm start the solver. For the Gurobi solver that we used, the random seeds and parallel computing are disabled. To provide additional clarity, we have added the following description to the revised manuscript:

	\medskip
 \textbf{Section IV.B:}
		
\color{blue}{``In cases where there is no computational time constraint or
a warm start has been provided, we have not observed any
uncertainty in the output of the solver — by no uncertainty,
we mean the solver provides the same solution in every run.
However, in the case a computational time limit exists without
any warm start, as illustrated in the first bar on the left plot
of Fig. 8, we have observed an uncertainty. Nevertheless, our
general conclusion remains valid that utilizing SVM-enabled
warm starts reduces the system cost, despite the existence of
such an uncertainty in certain situations.''}
\color{black}

 

 \item [3.6)]  \textbf{Comment:} \textit{``There are multiple occurrences of the typo "hing" which should be "hinge".''}
		
	\medskip
	\textbf{Response:} Sorry for the typos. We have corrected them.

\item [3.7)]  \textbf{Comment:} \textit{``In equation (7), the $\max$ should really be $\sup$ as it is known not to be attained (Example 2 in [2]) unless compactness of the sample set or concavity of the loss function is assumed
(neither of which seems to be the case here), or if the authors have alternative proofs.''}

	\medskip
	\textbf{Response:} Sorry for the typo. We have corrected it as
\medskip


  \textbf{Section IV.C:}
		
\color{blue}{``\begin{align} 
\min_{\mathbf{w},b}& \ \sup_{\mathbb{Q}\in \mathbb{B}_\rho(\hat{\mathbb{P}}_H)} \mathbb{E}^\mathbb{Q} \bigg[\mathbf{L}\big(y,(\mathbf{w}^\top \mathbf{x}+ b )\big)\bigg],
\end{align}''}
\color{black}

\textbf{Section IV.E:}
		
\color{blue}{``\begin{align} 
\min_{\boldsymbol\beta}& \sup_{\mathbb{Q}\in \mathbb{B}_\rho(\hat{\mathbb{P}}_H)} \mathbb{E}^\mathbb{Q} \Big[\mathbf{L}\Big(y,\sum_{h=1}^H   f(\mathbf{x},\mathbf{x}_h) \beta_h\Big)\Big].
\end{align}''}
\color{black}

\item [3.8)]  \textbf{Comment:} \textit{``Below equation (8), the term "norm 2 operator" is less standard and is thus suggested to be changed to simply "2-norm." It is also very weird to call (8) an "unconstrained quadratic programming problem" because is a piecewise linear function, so it is not smooth (and
hence not quadratic) or it needs linear constraints for a reformation with a quadratic objective function.''}
		
	\medskip
	\textbf{Response:} Thanks for the suggestion. We have changed ``norm 2 operator'' to ``2-norm''.  We fully agree with the Reviewer that (8) in the previous manuscript was an unconstrained problem that the first term is a piece-wise linear function whereas the second term is quadratic. To address the Reviewer's comment 3, we have omitted (8), but we have clarified formulation  \eqref{Linear_SVM_2}, which is written as a second-order cone problem. 
 \item [3.9)]  \textbf{Comment:} \textit{``Below equation (11) the notation $h=\{1,...,H\}$ and $k=\{1,...,H\}$ is suggested to
be changed into $h,k=\{1,...,H\}$.''}
		
	\medskip
	\textbf{Response:} Thanks. We have changed it as you suggested.
 
 \item [3.10)]  \textbf{Comment:} \textit{``Below equation (14), it is suggested to mention that the matrix $\boldsymbol f\in \R^{H \times H}$ is positive semidefinite, and include the explanation for the notation $\boldsymbol f^{\frac{1}{2}}\in \R^{H \times H}$ in (14a).''}
		
	\medskip
	\textbf{Response:} Thanks for suggestion. We have implemented it as follows:

 \medskip
  \textbf{Section IV.D:}
		
\color{blue}{``Note that $\boldsymbol f\in \R^{H \times H}$ is a positive semidefinite matrix that can be written as $\boldsymbol f=\boldsymbol f^{\frac{1}{2}} \boldsymbol f^{\frac{1}{2}}$. We use the Cholesky decomposition to find  $\boldsymbol f^{\frac{1}{2}}\in \R^{H \times H}$.''}
\color{black}
 
\item [3.11)]  \textbf{Comment:} \textit{``In the beginning of Section VI, it is suggested to include the source code repository link
directly in the text or in a footnote, instead using a citation.''}
		
	\medskip
	\textbf{Response:} Thanks. We followed this suggestion.

 \item [3.12)]  \textbf{Comment:} \textit{``In the experiment for the 6-bus system, the authors are using 4-fold cross validation on 1,000 samples. Any justification of the choice of 4 (instead of 5 or more) would strengthen the claim here.''}
		
	\medskip
	\textbf{Response:} 

Thanks for bringing up this comment, which has led us to notice a mistake. It is important to clarify that we employ cross-validation on the training dataset, not the testing dataset, which comprises 1,000 samples. Essentially, we fine-tune the parameters $\gamma$ in the Gaussian kernel function and the regularization term $\lambda$ through cross-validation on the training dataset, without referencing the test dataset, to prevent biasing the training process.

\medskip
In order to justify the selection of four folds, we conducted a sensitivity analysis in terms of the number of folds used in cross-validation. We varied the number of folds from 3 to 6 and observed that there is no notable change in the expected hinge loss. Specifically, we fount that the change is less than $0.1\%$ for both linear and kernelized SVM with regularization. Therefore, 4-fold is a good choice for cross validation. We have corrected the typo and added the following explanation to section VI.A of the revised manuscript:

\medskip
	
		\textbf{Section VI.A:}
		
\color{blue}{``To do so, we split training samples into $4$ equally sized subsets and then training the model on $3$ subsets, while validating its performance on the remaining subset. This process is repeated $4$ times, with each subset being used as the validation set once, and the other $3$ subsets being used for training. The performance metric used is the expected hinge loss of validation instances. Similarly, we regularize both linear and kernelized SVM classifiers by determining a value for $\lambda$, obtained by cross-validation too. Note that
we employ cross-validation on the training dataset, without using the test dataset, to prevent a biased training process.

\medskip
In order to justify the selection of four folds, we have conducted a sensitivity analysis regarding the number of folds used in cross-validation. We have varied the number of folds from $3$ to $6$ and observed that there is no notable change in the expected hinge loss. Specifically, we have found that the change is less than $0.1\%$ for both linear and kernelized SVM classifiers with regularization. By this, we have concluded $4$-fold is a reasonable choice for cross-validation.''}
 \color{black}



 %\begin{figure*} [t]
%\centering
%\begin{minipage}{.5\textwidth}
%  \centering
%  	\scalebox{1}{
%	\includegraphics[width=0.8\columnwidth]{Figures/crossvalidation-linear-cropped.pdf}
%	}
%\end{minipage}%
%\begin{minipage}{.5\textwidth}
%  \centering
%    	\scalebox{1}{
	%\includegraphics[width=0.8\columnwidth]{Figures/crossvalidation-rbf-cropped.pdf}
	%}
%\end{minipage}
%\caption{Sensitivity analysis on the number of folds for cross validation}
%\end{figure*}

  \item [3.13)]  \textbf{Comment:} \textit{``It is mentioned that "the MISOCP solver without warm start is very slow" for Figure 5. Some
further details on the reason (such as not able to find a feasible solution or just slow in
improving the bound) could provide more insights. Moreover, it would be more convincing if the authors could incorporate some modern techniques in the convex hull description of UC
decisions [3].''}

  \medskip
 \textit{[1] Shafieezadeh-Abadeh, Soroosh, Daniel Kuhn, and Peyman Mohajerin Esfahani.
"Regularization via mass transportation." Journal of Machine Learning Research 20, no. 103
(2019): 1-68.}

\medskip
\textit{[2] Mohajerin Esfahani, Peyman, and Daniel Kuhn. "Data-driven distributionally robust
optimization using the Wasserstein metric: performance guarantees and tractable
reformulations." Mathematical Programming 171, no. 1-2 (2018): 115-166.}

\medskip
\textit{[3] Pan, Kai, and Yongpei Guan. "Convex hulls for the unit commitment polytope." arXiv preprint arXiv:1701.08943(2017).}

		
	\medskip
	\textbf{Response:} 

 We have noticed that a considerable amount of the computational time is typically dedicated to obtaining a feasible solution with an objective value close to the dual bound (lower bound). This task of finding a feasible solution is commonly accomplished through generic primal heuristics embedded within the solver, which may be time-consuming. Modern solvers also offer an option for users to supply their own solutions, which can then be utilized by the solver to expedite the branch-and-cut process.

\medskip
It is worth noting that the solutions provided by the user do not necessarily have to be feasible. Advanced solvers are capable of repairing infeasible solutions using various heuristic techniques. This is actually a motivation for our proposed method. As an example, Fig. \ref{warm-start} illustrates the convergence of bounds for a random sample, comparing scenarios with and without the utilization of a warm-start approach. We have added the following clarification to Section VI.B of the revised manuscript: 
\begin{figure}[t]
    \centering
\includegraphics[width=0.7\columnwidth]{Figures/fig4.pdf}
    \caption{Convergence of bounds with and without warm-starting.}
    \label{warm-start}
\end{figure}


\medskip
	
		\textbf{Section VI.B:}
		
\color{blue}{``On the contrary, the MISOCP solver without warm start (first bar) is very slow, such that it could not solve the UC problem effectively in $700$ seconds, yielding a high optimality gap, and thereby a significant system cost. We observe that a significant portion of the running time is usually spent in finding a feasible solution. Therefore, the MISOCP solver warmly started by the predictions of other classifiers exhibits a performance in between.''}
 \color{black}

\medskip
It is indeed exciting to incorporate the convex hull description of binary decisions into the UC problem.
Thanks for suggesting the paper. However, we often use the convex hull description of UC decisions for pricing energy based on the UC problem [1]-[2], which fall beyond the scope of the current work. Although as a future research direction, we can investigate this idea. We have added the following suggestions as potential future works to Section VII of the revised manuscript:

\medskip
	
		\textbf{Section VII:}
		
\color{blue}{``Another direction for future work is to explore how to incorporate the convex hull description of UC decisions proposed
in [14], aiming to enhance the computational efficiency of
the UC problem as an expansion of this study. Additionally,
an intriguing direction for further investigation is to explore
methods for transfer learning to adapt to changes in the UC
problem, such as modifications in network topology, without
a need for retraining the binary classifier.''}

 \color{black}

	\medskip
[1] N. Azizan, and et al., "Optimal pricing in markets with nonconvex costs", Operations Research, vol. 68, no. 2, 2020.

	\medskip
[2] RP. O’Neill, and et al., "Efficient market-clearing prices in markets with nonconvexities", Eur. J. Oper. Res, 2005.

 \end{itemize}
	

==> comments.tex <==
% for underbar
\makeatletter
\def\munderbar#1{\underline{\sbox\tw@{$#1$}\dp\tw@\z@\box\tw@}}
\makeatother

\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{observation}{Observation}
\newtheorem{claim}{Claim}
%==================================
\newcommand{\peyman}[1]{{\color{blue} #1}}
\newcommand{\note}[1]{\textbf{{\color{red}(#1)}}}

%======================================
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{equation*}\begin{aligned}}
\newcommand{\eea}{\end{aligned}\end{equation*}}
\newcommand{\ds}{\displaystyle}
\newcommand{\independent}{\protect\mathpalette{\protect\independenT}{\perp}}
\newcommand{\R}{\mathbb{R}}

\newcommand{\Max}{\max\limits_}
\newcommand{\Min}{\min\limits_}
\newcommand{\Sup}{\sup\limits_}
\newcommand{\Inf}{\inf\limits_}
\newcommand{\Tr}[1]{\Trace \left[ #1 \right]}

\newcommand{\wh}{\widehat}
\newcommand{\mc}{\mathcal}
\newcommand{\mbb}{\mathbb}
\newcommand{\inner}[2]{\big \langle #1, #2 \big \rangle }
\newcommand{\cov}{\Sigma} % true covariance matrix


\newcommand{\trueP}{\p_0}
\newcommand{\empiP}{\wh{\p}}

\newcommand{\Struct}{\mc S} % structural set
\newcommand{\Ambi}{\mc P} % Ambiguity set
\newcommand{\AmbiGeneral}{\mc P}
\newcommand{\Data}{\wh{\mc Z}_N} % Data set
\newcommand{\DataKfold}{\wh{\mc D}}
\newcommand{\est}{\wh{X}} % DRO estimator for X
\newcommand{\estL}{\wh{\lambda}} % DRO estimator for lambda
\newcommand{\estx}{\wh{x}}
\newcommand{\DataOOS}{\wh{\Psi}_{N'}}


%\newcommand{\est}{X\opt}
%\newcommand{\estL}{\lambda\opt}
%\newcommand{\estx}{x\opt}



\newcommand{\defeq}{%
  \mathrel{\vbox{\offinterlineskip\ialign{%
    \hfil##\hfil\cr
    $\scriptscriptstyle\triangle$\cr
    %\noalign{\kern0ex}
    $=$\cr
}}}}

% Peyman's comments
\newcommand{\PSD}{\mathbb{S}_{+}} % the set of positive semi-definite matrices of dimension p
\newcommand{\PD}{\mathbb{S}_{++}} % the set of positive semi-definite matrices of dimension p
\newcommand{\Let}{\coloneqq}
\newcommand{\opt}{^\star}
\newcommand{\eps}{\varepsilon}
\newcommand{\ra}{\rightarrow}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Wass}{\mathds{W}}
\newcommand{\V}{\mathds{V}}
\newcommand{\Q}{\mbb{Q}}
\newcommand{\EE}{\mathds{E}}
\newcommand{\p}{\mbb P}
\newcommand{\FSFS}{\Theta}
\newcommand{\Z}{\mc Z}
\newcommand{\J}{\mc J}
\newcommand{\FS}{\Omega}

\newcommand{\m}{\mu}
\newcommand{\as}{\text{-a.s}}
\newcommand{\msa}{\wh{\m}}
\newcommand{\covsa}{\wh{\cov}}
\newcommand{\M}{\mc M}











==> style.tex <==
\usepackage{float,graphicx,epstopdf}
\usepackage{bbm}  % for the indicator function \mathbbm{1}
\RequirePackage[reqno]{amsmath}
\usepackage{cases}
\usepackage{url}


% ==== Peyman style ======================
\usepackage[usenames, dvipsnames]{color}
\definecolor{darkblue}{rgb}{0.0, 0.0, 0.45}

\usepackage[colorlinks	= true,
raiselinks	= true,
linkcolor	= MidnightBlue, %darkblue, %
citecolor	= Mahogany,
urlcolor	= ForestGreen,
pdfauthor	= {},
pdftitle	= {},
pdfkeywords	= {},
pdfsubject	= {},
plainpages	= false]{hyperref}

\usepackage{dsfont,amssymb,amsmath,subfigure, graphicx,enumitem} %,etaremune,savesym}
\usepackage{amsfonts,dsfont,mathtools, mathrsfs,amsthm,fancyhdr} 
\usepackage[amssymb, thickqspace]{SIunits}
%\usepackage{algorithm,algorithmicx}

% ================== Margins & Layout =================================
\addtolength{\voffset}{0cm} 
\addtolength{\textheight}{1cm} 
\addtolength{\hoffset}{-2cm}
\addtolength{\textwidth}{4cm}

\setlength{\parskip}{1mm}
\linespread{1.12}

%======== Theorem Environments ===============================
\renewcommand\thesection{\arabic{section}}
\renewcommand\thesubsection{\thesection.\arabic{subsection}}

% ====== Change section title ===============================
\makeatletter
\def\@settitle{\begin{center}%
		\baselineskip14\p@\relax
		\normalfont\LARGE\scshape\bfseries
		%\uppercasenonmath\@title
		\@title
	\end{center}%
}
\makeatother
\makeatletter

\def\subsection{\@startsection{subsection}{2}%
	\z@{.5\linespacing\@plus.7\linespacing}{.5\linespacing}%
	{\normalfont\large\bfseries}}

\def\subsubsection{\@startsection{subsubsection}{3}%
	\z@{.5\linespacing\@plus.7\linespacing}{.5\linespacing}%
	{\normalfont\itshape}}



